Linear convergence in time-varying generalized Nash equilibrium problems

We study generalized games with full row rank equality constraints and we provide a strikingly simple proof of strong monotonicity of the associated KKT operator. This allows us to show linear convergence to a variational equilibrium of the resulting primal-dual pseudo-gradient dynamics. Then, we propose a fully-distributed algorithm with linear convergence guarantee for aggregative games under partial-decision information. Based on these results, we establish stability properties for online GNE seeking in games with time-varying cost functions and constraints. Finally, we illustrate our findings numerically on an economic dispatch problem for peer-to-peer energy markets.

==> ArXiv submission/macros.tex <==
%Packages
% \usepackage{generic}
 \usepackage{amsmath, amssymb, bbm, xspace}
 \usepackage{amsfonts,mathrsfs}
 \usepackage{mathtools}
 \usepackage{color}
 \usepackage{graphicx}
 \usepackage{epsfig}
 \usepackage{algorithm}
 \usepackage{algorithmicx}
 \usepackage[acronym]{glossaries}
 \usepackage{subfigure}
 \usepackage{cancel}
 \usepackage{empheq}
 \usepackage{placeins}
 \let\labelindent\relax
 \usepackage{enumitem}
 \usepackage{textgreek}
 \usepackage{mathbbol}
 \usepackage{stackengine}
\usepackage{placeins}
\usepackage{dblfloatfix}
\usepackage{cancel}

 %Commands
 \def\QEDhereeqn{\eqno\let\eqno\relax\let\leqno\relax\let\veqno\relax\hbox{\QED}}
 \def\QEDopenhereeqn{\eqno\let\eqno\relax\let\leqno\relax\let\veqno\relax\hbox{\QEDopen}}
 \newcommand{\bs}{\boldsymbol}
 \newcommand{\mc}{\mathcal}
 \renewcommand{\emph}{\textit}
 \newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
 \newcommand{\0}{\bs 0}
 \def\1{{\bs 1}}
 \def\argmin{\mathop{\rm argmin}}
\def\min{\mathop{\rm min}}
 \newcommand{\col}{\mathrm{col}}
 \def\diag{\mathop{\hbox{\rm diag}}}
 \def\interior{\mathop{\hbox{\rm int}}}
 \newcommand{\proj}{\mathrm{proj}}
 \def\dom{\operatorname{dom}}
 \def\R{\mathbb{R}}
 \def\N{\mathbb{N}}
 \def\I{\mc{I}}
 \def\i{{i\in\mc{I}}}
 \def\neigi{\mc{N}_i}

 % Symbols
 \DeclareSymbolFontAlphabet{\mathbbm}{bbold}
 \DeclareSymbolFontAlphabet{\mathbb}{AMSb}%
 \def\h{\mathbbm{x}^\star}
 \stackMath
	 \newcommand\tsup[2][2]{%
	 	\def\useanchorwidth{T}%
	 	\ifnum#1>1%
	 	\stackon[-.5pt]{\tsup[\numexpr#1-1\relax]{#2}}{\scriptscriptstyle\sim}%
	 	\else%
	 	\stackon[.5pt]{#2}{\scriptscriptstyle\sim}%
	 	\fi%
	 }

 %Glossaries
\makeglossaries
\newacronym{KKT}{KKT}{Karush--Kuhn--Tucker}
\newacronym{ADMM}{ADMM}{alternating direction method of multipliers}
\newacronym{OPF}{OPF}{optimal power flow}
\newacronym{OPFP}{OPFP}{optimal power flow problem}
\newacronym{NUM}{NUM}{network utility maximization}
\newacronym{LMI}{LMI}{linear matrix inequality}
\newacronym{BMI}{BMI}{bilinear matrix inequality}
\newacronym{LM}{LM}{Lyapunov-Metzler}
\newacronym{SDP}{SDP}{semidefinite programming}
\newacronym{LTI}{LTI}{linear time invariant}
\newacronym{MJLS}{MJLS}{Markov jump linear system}
\newacronym{PID}{PID}{proportional-integral-derivative}
\newacronym{PPA}{PPA}{proximal-point algorithm}
\newacronym{PPPA}{PPPA}{preconditioned proximal-point algorithm}
\newacronym{PPP}{PPP}{preconditioned proximal-point}
\newacronym{NE}{NE}{Nash equilibrium}
\newacronym{GNE}{GNE}{generalized Nash equilibrium}
\newacronym{v-GNE}{v-GNE}{variational GNE}
\newacronym{ISS}{ISS}{input-to-state stability}



 %Crossref
 \makeatletter \let\cl@part\relax \makeatother
 \usepackage{nohyperref}
 \usepackage[capitalize]{cleveref}
  \let\k\relax
 \def\k{{k \in \N}}  %there is some conflict with this command
 \usepackage{letltxmacro}

 \crefname{thm}{Theorem}{Theorems}
 \crefname{lem}{Lemma}{Lemmas}
 \crefname{cor}{Corollary}{Corollaries}
 \crefname{rem}{Remark}{Remarks}
 \crefname{alg}{Algorithm}{Algorithm}
 \crefname{figure}{Figure}{Figures}
 \crefname{assumption}{Assumption}{Assumptions}
 \crefname{corollary}{Corollary}{Corollaries}
\crefname{proposition}{Proposition}{Propositions}
\crefname{problem}{Problem}{Problems}
\crefname{example}{Example}{Examples}
\crefname{definition}{Definition}{Definition}
\crefname{condition}{C}{C}


 \crefname{thmlisti}{Theorem}{Theorem}
 \crefname{lemlisti}{Lemma}{Lemma}
 \crefname{asmlisti}{Assumption}{Assumptions}

 \newlist{thmlist}{enumerate}{1}
 \setlist[thmlist]{label=(\roman{thmlisti}), ref=\thethm(\roman{thmlisti}),noitemsep}
 \newlist{lemlist}{enumerate}{1}
 \setlist[lemlist]{label=(\roman{lemlisti}), ref=\thelem(\roman{lemlisti}),noitemsep}
 \newlist{asmlist}{enumerate}{1}
 \setlist[asmlist]{label=(\roman{asmlisti}), ref=\theassumption(\roman{asmlisti}),noitemsep,nosep,leftmargin=*} %wide=0pt


 \newtheorem{lemma}{Lemma}
 \newtheorem{theorem}{Theorem}
 \newtheorem{remark}{Remark}
 \newtheorem{assumption}{Assumption}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{condition}{C \hspace{-0.7em}} %\newenvironment{proof}[1][Proof]{\noindent\textbf{#1.} }{\ \rule{0.5em}{0.5em}}


%Custom
\def\M{\mc{M}}
\def\Mp{\mc{M}_+}
\def\D{\mc{D}}
\def\C{\mc{C}}
\def\ms{{\hspace{-0.25em}}}
\def\W{\mc{W}}
\def\Pit{\tilde P_i}
\def\Pjt{\tilde P_j}
\def\Pbs{\bs{P}_{\ms -i}}
\def\Pibs{\bs{\pi}_{ -i}}

\def\Acl{A^{\textrm{cl}}}
\def\Acli{{A^{\textrm {cl}}_i}}

\usepackage{etoolbox}
\patchcmd{\smallmatrix}{\thickspace}{\kern.5em}{}{}
\newenvironment{smallbmatrix}
  { \left[\begin{smallmatrix}}
  {\end{smallmatrix}\right]}

\usepackage{caption}% http://ctan.org/pkg/caption
\captionsetup[table]{format=plain,labelformat=simple,labelsep=period}
\usepackage{booktabs}
\usepackage{multirow}

\def\Fmc{\mc{F}}
\def\H{\mc{H}}
\def\zer{\operatorname{zer}}
\def\gra{\operatorname{gra}}
\def\Fbs{\bs{F}}
\def\Fa{\Fmc_{\alpha}} 
\def\Rmc{\mc{R}}
\def\Fop{\Rmc^\top \Fbs}
\def\condref#1{C\ref{#1}}
\def\subd#1{\partial_{#1}}
\def\grad#1{\nabla_{#1}}
\def\x{\bs{x}}
\def\sol{\mc{S}}
\def\X{\Omega}
\def\Lbs{\bs{L}}
\def\dom{\operatorname{dom}}
\def\A{\mc{A}_{\alpha}}
\def\Ak{\mc{A}_{\alpha^k}}
\def\Id{\operatorname{Id}}
\def\Wbs{\bs{W}}
\def\nc{\mathrm{N}}
\def\res{\mathrm{J}}
\def\ubs{\bs{u}}
\def\fix{\operatorname{fix}}
\def\y{\bs{y}}
\def\pal{_{\scriptscriptstyle \parallel}}
\def\perr{_{\scriptscriptstyle \perp}}
\def\xbsstar{\x^\star}
\def\Xbs{\bs{\Omega}}
\def\ybs{\bs{y}}
\def\Lbs{\bs{L}}

\DeclareSymbolFont{myletters}{OML}{ztmcm}{m}{it}
\DeclareMathSymbol{\uplambda}{\mathord}{myletters}{"15}

